Task Facet Learning: A Structured Approach to Prompt Optimization

Given a task in the form of a basic description and its training examples, prompt optimization is the problem of synthesizing the given information into a text prompt for a large language model. Humans solve this problem by also considering the different facets that define a task (e.g., counter-examples, explanations, analogies) and including them in the prompt. However, it is unclear whether existing algorithmic approaches, based on iteratively editing a given prompt or automatically selecting a few in-context examples, can cover the multiple facets required to solve a complex task. In this work, we view prompt optimization as that of learning multiple facets of a task from a set of training examples. We exploit structure in the prompt optimization problem and break down a prompt into loosely coupled semantic sections. The proposed algorithm, UniPrompt, (1) clusters the input space and uses clustered batches so that each batch likely corresponds to a different facet of the task, and (2) utilizes a feedback mechanism to propose adding, editing or deleting a section, which in turn is aggregated over a batch to capture generalizable facets. Empirical evaluation on multiple datasets and a real-world task shows that prompts generated using \shortname{} obtain higher accuracy than human-tuned prompts and those from state-of-the-art methods. In particular, our algorithm can generate long, complex prompts that existing methods are unable to generate. Code for UniPrompt is available at https://aka.ms/uniprompt.

==> formulation.tex <==
\section{Text-gradient based prompt optimization: Challenges, Insights} 
\label{sec:formulation}
State-of-the-art prompt optimization methods such as
ProTeGi \citep{pryzant2023automatic} and TextGrad \citep{houtextgrad} iteratively optimize the prompt for a given task. They adopt the following procedure at a high-level: (1) start with an initial prompt and a training dataset of $\langle$question, answer$\rangle$ pairs for the task, (2) randomly sample from the questions wrongly answered by the current prompt to form a batch, (3) use an expert LLM to obtain feedback on the random batch, (4) apply the feedback to the prompt. This procedure is illustrated in Figure \ref{fig:main} [Left]. 
In this section, we study when such optimization is feasible and what may be the issues with current prompt optimization procedures. 


\subsection{When is directional text optimization feasible?} 
Consider the class of sequential algorithms as outlined above. %that decide the next prompt based on all previous $\langle$prompt, output accuracy$\rangle$ pairs and a fixed task-specific training set that provides (labelled) input-output pairs for the task. We do not have access to the gradients, hence it is a zeroth-order optimization problem --- 
The objective is to improve the accuracy of a given (black-box) \textit{solver LLM} $f:\mathcal{X} \rightarrow \mathbb{R}$ that takes as input a prompt $\mathbf{x} \in \mathcal{X}$ and outputs the average accuracy on a validation set $D_v$. 
%Previous work has shown that LLMs can be  brittle to their input: changing the prompt slightly can create a significant difference in performance~\citep{zhuo2023robustness}. %To understand whether optimization algorithms may work, it is important to understand how the surface of $f$ looks. If $f$ is brittle everywhere to small changes, then it is unclear if gradient-based optimization can perform any better than random search over prompts (such as in \cite{APE}). On the other hand, if the change in $f$ given small changes to the input prompt is bounded, then optimization algorithms can hope to perform significantly better than random search. 
Since the set of prompts is combinatorially large, we assume that all prompts can be embedded in a vector space such that distance between two prompts in the space correspond to their semantic similarity. %Thus, each prompt $\mathbf{x}$ can be expressed as a vector in $\mathbb{R}^p$. 
The prompt optimization problem can be written as $\arg \max_{\mathbf{x} \in \mathcal{X}} f(\mathbf{x}; D_v)$.

% We do not have access to the gradients, hence it is a zeroth-order optimization problem. For optimization, we consider the class of sequential algorithms that decide the next prompt  based on all previous $\langle$prompt, output accuracy$\rangle$ pairs and a fixed task-specific training set that provides (labelled) input-output pairs for the task. 


% \subsection{Is directional optimization feasible?}
% \label{sec:lipschitz}
% Previous work has shown that LLMs can be  brittle to their input: changing the prompt slightly can create a significant difference in performance~\cite{zhuo2023robustness}. To understand whether optimization algorithms may work, it is important to understand how the surface of $f$ looks. If $f$ is brittle everywhere to small changes, then random search over prompts (such as in \cite{APE})  may be a competitive method; it is unclear whether optimization can help. On the other hand, if the change in $f$ given small changes to the input prompt is bounded, then optimization algorithms can hope to perform significantly better than random search. 

Previous work has shown that LLMs can be  brittle to their input: changing the prompt slightly can create a significant difference in performance~\citep{zhuo2023robustness}.
We want to understand if the optimization problem is well-conditioned. Typically, conditioning can  be determined by the Hessian. However, since $f$ is black-box, we approximate it by measuring sensitivity, or more specifically, Lipschitz continuity near the optimal solution. Based on prior work on defining continuity of neural networks~\citep{nori}, we use a probabilistic notion. 

\begin{definition}[Probabilistic Lipschitz Continuity~\citep{nori}]
\label{def:k_delta_lipschitz}
Given a probability distribution over inputs $\mathcal{X}$, $r \geq 0$, and a distance measure $d$ such as $\ell_1$ or $\ell_2$ norm, a function $f: \mathcal{X} \rightarrow \mathbb{R}$ is $(L, \epsilon)$-probabilistically Lipschitz with constant $L \geq 0$, if
\begin{align}
    \Pr_{\mathbf{x},\mathbf{x}' \sim \mathcal{X}}[&\operatorname{d}(f(\mathbf{x}),f(\mathbf{x}')) \leq L \cdot \operatorname{d}(\mathbf{x},\mathbf{x}') \nonumber \\
    &|  \ \operatorname{d}(\mathbf{x},\mathbf{x}') \leq r] \geq 1-\epsilon .
\end{align}
\end{definition}



Note the focus on small changes in input through the parameter $r$. Intuitively, the Lipschitz property bounds the maximum change in $f$ given a small change in input prompt. Typically, the lower bound of error for any sequential optimization algorithm over $f$ is directly proportional to the Lipschitz constant $L$~\citep{malherbe2017global}. Therefore, for faster convergence, it is desirable to have a low $L$, especially near the optimal solution. 

Empirically, we estimate $L$ by sampling task-relevant prompts so that they are close to the optimal solution. Then we make small changes to the prompt such that the semantic meaning stays the same and measure the change in $f$ (See Appendix \ref{app:sec2.1} for experimental details). We show the change in $f$ per change in input for GPT4 and GPT3.5 models in Figure~\ref{fig:motivation} for the Ethos, GSM8K and MedQA datasets. 
% \naga{need to update this para once fig is finalized.}%~\citep{pryzant2023automatic, ethos_cite_1, ethos_cite_2,ethos_cite_3, ethos_cite_4}.
Assuming $\epsilon=0.05$, probabilistic Lipschitz constant $L$ for GPT4 is $<1$, whereas it is higher for GPT3.5. Thus, as the model sizes increases, the probabilistic Lipschitz constant decreases. So:%,, indicating that larger models are more robust to small changes and thus amenable to optimization algorithms. 
% For Llama, the absolute change in accuracy ranges between 0.33 to 0.54, indicating a 63\% change in accuracy even across prompts with the same semantic meaning. In contrast, the relative change in accuracy for GPT-3.5 and GPT-4 is 6\% and 4\% respectively 

\textbf{Observation 1: Larger models are more amenable to prompt optimization.} 
% \begin{figure*}
%     \centering
%     \begin{subfigure}[b]{0.325\textwidth}
%         \centering
%         \includegraphics[width = \linewidth]{Images/Lip_ethos.png}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.325\textwidth}
%         \centering
%         \includegraphics[width = \linewidth]{Images/Lip_GSM8K.png}
%     \end{subfigure}
%       \begin{subfigure}[b]{0.325\textwidth}
%         \centering
%         \includegraphics[width = \linewidth]{Images/Lip_Medqa.png}
%     \end{subfigure}
%     \caption{Estimating (probabilistic) Lipschitz constant of models (Definition \ref{def:k_delta_lipschitz}) on (left) Ethos (middle) GSM8K and (right) MedQA datasets for GPT-4 and GPT-3.5 models.}
% \label{fig:motivation}    
% \end{figure*}

\subsection{Can we do better than random batching?}
Batching is standard in gradient-based optimization to obtain robust gradients. Text-gradient based prompt optimization techniques such as ProTeGi \citep{pryzant2023automatic} and TextGrad \citep{houtextgrad} also adopt batching by randomly sampling from training examples where the solver LLM made a mistake. In the early iterations of optimization, there can be many such examples --- is random batching sufficient to get meaningful feedback (i.e., the text gradient) from the expert model?   

To investigate this, we consider the Ethos dataset where the task is to classify text as hate speech or not. We start with a basic task description as the prompt, ``\textit{Is the following text hate speech (1) or not (0)?}'', run it with GPT-3.5 on 200 examples, and then provide random batches of incorrect predictions to GPT-4 to identify prompt edits. GPT-4 is prompted to provide edits to the current prompt such that the errors are minimized. With a random batch, the feedback obtained is relevant for the task, but fails to identify specific concepts. Example feedback include, 

\begin{quote}
\textit{The instruction should include a clear definition of hate speech...}

\textit{The instruction should include examples of hate speech, guidance on identifying hate speech...}
\end{quote}

Instead, if we cluster the incorrect examples (see Section~\ref{sec:clustering}) and create clustered batches, we obtain the following feedback.
\begin{quote}
\textit{The instruction should include..potential harm or violence implied, as well as any discriminatory or derogatory language used...towards a particular religious group. }

\textit{The instruction should include ...think about the impact of the statement on the targeted individual or group.}

\textit{The instruction should include...language that prompts hatred or discrimination towards a particular gender.}
\end{quote}

The first feedback captures the religious and harm-based aspect of hate speech whereas the second captures the aspect of measuring impact on the targeted entity. This case-study suggests that  the same LLM is able to identify different facets due to clustered batches. 

\textbf{Observation 2: Clustered-batching improves the quality of text gradients.} 

\subsection{Can we learn a generalizable prompt from a limited set of examples?}

The optimal prompt should consider all the aspects of the task. So, any prompt optimization algorithm (or a human prompt engineer for that matter) may have to exhaustively sample from the data distribution in many real-world scenarios. In practice, however, we have access only to a limited number (a few hundreds) of training examples (as it requires exhaustive manual labeling).  We present such a case study in Section \ref{sec:queryintent} that arises in search and recommendation pipelines. The task is to infer if two search queries share identical intent or not. Here, the notion of ``identical intent'' is captured implicitly in the human-labeled query-pairs. 

In this data-constrained setting, consider the standard in-context learning~\citep{ICL}, where the prompt is composed of a simple task description and a set of labeled examples from the task. There are many ways in the literature to select examples for in-context learning, including random sampling and k-nearest neighbors. In our setting, perhaps it would be beneficial to consider the marginal utility of examples \citep{zhang2022active,gupta2023coverage}, i.e., add examples where the model fails rather than ones where the model already succeeds (see Table \ref{tab:length} in Appendix). This suggests that one could use a greedy algorithm for iteratively optimizing the prompt by finding failing examples and adding to the prompt. \textit{But would such a procedure converge to a good solution that generalizes to unseen examples?}

% We can view $f(\mathbf{x})$ as a set function over the examples (that compose $\mathbf{x}$). A natural property to examine is \textit{submodularity} (where greedy optimization provably converges to a good solution under some conditions \cite{krause2014submodular}), i.e., the property of diminishing marginal utility of examples. The marginal utility of adding an example $e$ to the few-shot prompt corresponding to a set of examples $A$ is $\Delta_A = f(A \cup \{e\}) - f(A)$. Let $B \subset A$ denote a subset of $A$.  We define $f_{\text{fewshot}}$ to be the validation accuracy of GPT-3.5 using few-shot prompts on the Ethos dataset (see Section \ref{sec:datasets}). In Figure \ref{fig:motivation} (b), we show the distribution of diminishing marginal utilities for $f_{\text{fewshot}}$ (light blue), i.e., we sample multiple $A, B$ sets of examples from the dataset and compute $\Delta_B  - \Delta_A$, which is expected to be non-negative for submodular functions. As we see, the marginal utility differences are nearly uniformly random in $[-0.01, 0.01]$, indicating that there is no submodularity structure to $f_{\text{fewshot}}$.

As we saw in the example above, such a procedure based on incorrect examples does provide specific facets, such as being focused on religious or gender groups. However, adding any of these texts directly to the prompt may be too specific and may miss out on other groups that may be targeted by hate speech (e.g., groups based on ethnicity). A procedure to aggregate the feedback may encourage the expert LLM to propose edits that are generalizable. In this example, we provide the three feedback texts above to the same expert LLM and ask it to summarize them into a single feedback. We obtain, 
\begin{quote}
\textit{The instruction should...consider whether the statement contains discriminatory, derogatory, or violent language that promotes hatred or harm towards a particular group, such as based on religion and gender.}
\end{quote}

As can be seen above, the summarized feedback captures the essence of the individual feedback texts and generalizes it to any group. A two-tier feedback, therefore, can help in distilling important aspects of the task implicit in the examples, rather than directly use or rephrase the (limited) examples. 

%We hypothesize that there are a small number of \textit{facets} that collectively define a task, which can be discovered by inspecting a representative set of examples from the data distribution. Consider the task of tagging hate speech. Identifying intent to harm, recognizing general aggression versus targeted hate, and differentiating hate from other objectionable content are some facets of the task that can be captured as sections in the prompt (like how a human prompt engineer would). 

%Can we discover the task facets using iterative text-gradient based optimization methods? 

%\textit{The prompt optimization problem can now be posed as one of inferring the facets of a task from a set of training examples.} In the following section, we propose a method that iteratively learns the facets of the task as sections of the prompt. 

%We ask whether there is submodularity structure in adding different facets (text sections) to a prompt, compared to adding in-context examples. 
% The answer to this question depends on multiple factors: (1) what are the contents of the sections and how are they generated?; (2) how does  $f(\mathbf{x})$ behave w.r.t. the sections that make up the prompt $\mathbf{x}$?


\textbf{Observation 3: Two-tier feedback helps learn generalizable facets in prompts.} 

% \subsection{Can higher-order abstractions of task examples help prompt optimization?}
% \label{sec:submodularity}
% Consider in-context learning~\citep{ICL}, where the prompt $\mathbf{x}$ is composed of a simple task description and a set of labeled examples from the task. The optimal prompt should consider all the aspects of the task which can only be discovered by exhaustively looking at the examples. But, in practice, we are constrained by (a) availability of a limited number of training examples, (b) prompt size. It is beneficial for in-context learning to consider the marginal utility of examples \cite{zhang2022active,gupta2023coverage}. For instance, it would help to add examples where the model fails rather than ones where the model already succeeds (see Table \ref{tab:length} in Appendix). This suggests that one could use a greedy algorithm for iteratively optimizing the prompt by finding failing examples and adding to the prompt. \textit{But would such a procedure converge to a good solution?}


% We can view $f(\mathbf{x})$ as a set function over the examples (that compose $\mathbf{x}$). A natural property to examine is \textit{submodularity} (where greedy optimization provably converges to a good solution under some conditions \cite{krause2014submodular}), i.e., the property of diminishing marginal utility of examples. The marginal utility of adding an example $e$ to the few-shot prompt corresponding to a set of examples $A$ is $\Delta_A = f(A \cup \{e\}) - f(A)$. Let $B \subset A$ denote a subset of $A$.  We define $f_{\text{fewshot}}$ to be the validation accuracy of GPT-3.5 using few-shot prompts on the Ethos dataset (see Section \ref{sec:datasets}). In Figure \ref{fig:motivation} (b), we show the distribution of diminishing marginal utilities for $f_{\text{fewshot}}$ (light blue), i.e., we sample multiple $A, B$ sets of examples from the dataset and compute $\Delta_B  - \Delta_A$, which is expected to be non-negative for submodular functions. As we see, the marginal utility differences are nearly uniformly random in $[-0.01, 0.01]$, indicating that there is no submodularity structure to $f_{\text{fewshot}}$.  

% A recurring theme~\citep{structure2, structure3} in the prompts that humans engineer is to organize task information in ``sections'' (introduction, context, etc.), treating prompt like a structured document. When humans engineer a prompt, they do it systematically by editing specific sections of the prompt. We hypothesize that there are a small number of \textit{facets} that collectively define a task, which can be discovered by inspecting a representative set of examples from the data distribution. Consider the task of tagging hate speech. Identifying intent to harm, recognizing general aggression versus targeted hate, and differentiating hate from other objectionable content are some facets of the task. We ask whether there is submodularity structure in adding different facets (text sections)  to a prompt, compared to adding in-context examples. 
% The answer to this question depends on multiple factors: (1) what are the contents of the sections and how are they generated?; (2) how does  $f(\mathbf{x})$ behave w.r.t. the sections that make up the prompt $\mathbf{x}$?



% Figure \ref{fig:motivation} (b) shows the distribution of marginal utility differences for $f_{\text{facets}}$ (dark blue), i.e., we sample multiple $A, B$ sets of \textit{facets} (i.e., short sections) that are generated using a Llama2-13B model, and compute $\Delta_B  - \Delta_A$ (defined as above, but the added element $e$ is now a section) using GPT-3.5 as the solver LLM (See Appendix \ref{app:sec2.2} for experimental details). We see that the diminishing marginal returns property largely holds for $f_{\text{facets}}$, unlike in the case of $f_{\text{fewshot}}$. This suggests that greedy strategies for prompt optimization problem over sections could work --- but this crucially relies on how we generate the sections themselves.   


% \textit{The prompt optimization problem can now be posed as one of inferring the facets of a task from a set of training examples.} In the following section, we propose a method that iteratively learns the facets of the task as sections of the prompt. 
